QEHeat: An open-source energy flux calculator for the computation of heat-transport coefficients from first principles

We give a detailed presentation of the theory and numerical implementation of an expression for the adiabatic energy flux in extended systems, derived from density-functional theory. This expression can be used to estimate the heat conductivity from equilibrium ab initio molecular dynamics, using the Green-Kubo linear response theory of transport coefficients. Our expression is implemented in an open-source component of the QE suite of computer codes for quantum mechanical materials modelling, which is being made publicly available.

==> parameter_tuning.tex <==
We show the stability and convergence properties of a \qeheat\ calculation on a snapshot of 125 water molecules. 
%give some tips to choose and control the parameters of a typical \qeheat\ calculation. 
%One is the self-consistency (scf) convergence threshold, $econv$, a standard parameter of QE scf computation, the other is the small timestep $dt$ used in the computation of the derivative using the finite difference, see \cref{eq:generic} in  \cref{sec:code_structure}, and it is a parameter specific of QE-Heat.
\cref{fig:3p_econv} reports a scaled version of the three Cartesian components of the MUB energy flux $J_{i}(dt),i \in \{x,z,y\}$, as a function of the time-discretization parameter $dt$. The $x-$axis is in units of the Car-Parinello MD simulation timestep, indicated with $\Delta t$. For each Cartesian coordinate, the behaviour of the error $( J_{i}(dt)- J_{\text{REF},i} )/ J_{\text{SCALE}}$, considering a reference and scale values, is reported, thus showing possible non-linear contributions due to the choice of a large $dt$. The reference value $J_{\text{REF},i}$ is evaluated for each coordinate at the smallest value of $dt$ available and $J_{SCALE} = |\bm J_{\text{REF}}|$. %\AMcancel{ The symbols $J_{dt, i}$ refers to a component of the MUB flux computed with the corresponding $dt$ in the $x$-axis, the symbols with tildas, instead, refers to the reference converged MUB flux, in the example taken to be with $dt/\Delta t=0.66$.}
\cref{fig:3p_econv} shows the presence of small non-linear effects for higher values of $dt$, and that, at least for the presented system, nonlinear effects do not take off substantially up to $dt=2\Delta t$. At this value of $dt$, even reducing it by a factor of 10 would change the component of the current by less than 1\%, a negligible error given that a typical value of the thermal transport coefficient has an accuracy of 10\% \cite{Marcolongo2014,Bertossa2019,Grasselli2020}. Moreover $dt=2\Delta t$ would be beneficial in an on-the-fly computation, allowing to reuse the same wavefunctions computed in the MD simulation, neglecting the need for the recomputation of the scf cycles. 
The results presented in this section have been computed with a rather stringent value of the self-consistency (scf) convergence threshold $econv$, $10^{-14}~$Ry, thus leading to an errorbar due to the precisions of the wavefunctions which is negligible on the scale of figure \cref{fig:3p_econv}. This negligible errorbar was evaluated for each component starting from the variance of the MUB flux provided by the testing tool of \qeheat\, which averages many fluxes obtained from different initial random wavefunctions, and than applying standard error propagation to compute the final errorbar in \cref{fig:3p_econv}. In order to save computational time, one would like to relax such a small value of $econv$, at the expense of increasing slightly the error bar and optimize the bias versus variance tradeoff. Note that, as discussed in \ref{sec:rdt_ren_2p},  at a fixed value of $econv$ the variance of the MUB estimator decreases with $dt$. Thus, it favourable, in order to control numerical noise, to choose $dt$ as large as possible, as long as the bias, discussed at the beginning of this section and introduced by nonlinear effects, is negligible.  We suggest to fix $dt=2\Delta t$ from the previous analysis and than optimize the value of the scf threshold for convergence $econv$, choosing it large enough to save computational cost, while keeping at the the same time a good accuracy of the resulting heat flux. An optimal choice in this case was $econv$ equal to $10^{-8}$Ry, which still provides a small variance (percentage error, see also \ref{sec:rdt_ren_2p}). In the next section we provide a more detailed evidence of the effect of $dt$ and $econv$ on the final computation of a heat transport coefficient.
It is worth to mention that we analyzed numerically also the effect of the energy cut-off on the stability w.r.t. $dt$ and we did not register any relevant behaviour. Thus it is not shown in the present work, and we adopted, and we suggest an user to adopt, the same cut-off of the MD simulation, $85~$Ry in the presented example. 
%\DTcancel{\cref{fig:3p_econv} shows, as expected, that higher values of $econv$ generate values of the current less stable with $dt$, in particular for small values of $dt$ where the computation is more sensitive to noise. Thus, the code can reach any chosen accuracy and stability, changing the parameter of the computation accordingly. 
%To test and prove further the stability of the MUB current as a function of $dt$, we used the testing feature already presented in \cref{sec:UsageBenchmarks} to compute an estimate of the statistical uncertainty, averaging many fluxes obtained from different initial random wavefunctions. \cref{fig:3p_err} shows the percentage error of the $x$-component of the flux for a specific snapshot of 125 molecule of water as function of $dt$. Each line corresponds to a different value of $econv$, even though the behaviour is similar. It is clear that increasing $econv$ increases the statistical error by some order of magnitude, three order from $10^{-14}$ to $10^{-08}$. It must be stated that the errors in \cref{fig:3p_err} do not include the effect of the non-linearity due to a too large $dt$, which can be seen, for example, in the lower panel of \cref{fig:3p_econv}.}
%\DTcancel{To conclude the section, we give some thought about optimal values of $dt$. From \cref{fig:3p_econv} we can clearly see that $dt=\Delta t$ it is pretty optimal, in fact, fixing $econv=10^{-14}$ for stability, even reducing $dt$ by a factor of 10 or 100 will change the component of the current by less than 1\%, a negligible error given that a typical value of the thermal transport coefficient has an accuracy of 10\%} \cite{Marcolongo2014,Bertossa2019,Grasselli2020}\DTcancel{.
%Using $dt=\Delta t$ allows, as we showed, to use less stringent values of $econv$ to obtain lower computational times. Moreover, it will be beneficial in an on-the-fly computation, allowing to reuse the same wavefunctions computed in the MD simulation, neglecting the need for the recomputation of the scf cycles. 
%It is worth to mention that we, also, studied the effect of the energy cut-off on the $dt$ stability and we did not register any relevant behaviour. Thus it is not shown in the present work, and we adopted, and we suggest an user to adopt, the same cut-off of the MD simulation, $85~$Ry in the presented example. }

%\begin{figure}[bth]
%    \centering
%    \includegraphics[width=0.8\textwidth]{figure_different_econv_nuovo.pdf}
%    \caption{\DTnote{Stefano?} The behaviour of $\frac{\delta J_i}{\Tilde{J}} $ as a function of the timestep $dt$ used in the 3-point derivative for a snapshot of water. Where $\delta J_i = J_{dt, i}- \Tilde{J}_i$, $\Tilde{J} = \sqrt{\Tilde{J}_x + \Tilde{J}_y +\Tilde{J}_z}$ and $i=x,y,z$. \AMnote{Proposta notazione diversa nel testo}The symbols $J_{dt, i}$ refers to a component of the MUB flux computed with the $dt$ reported in the $x$-axis, the symbols with tildas refers to the reference converged MUB flux, in the example taken to be with $dt/\Delta t=0.66$. The $x$-axis is in units of the simulation step $\Delta t$. The picture shows that the code can handle correctly even small values of $dt$. At the same time, it shows that the non-linear effects due to high values of $dt$ are present but, at least in the presented case, negligible, allowing a $dt=2\Delta t$.} 
%    \label{fig:3p_econv}
%\end{figure}

%\begin{figure}[bth]
%    \centering
%    \includegraphics[width=0.8\textwidth]{figure_different_econv_n%uovo.pdf}
%    \caption{The behaviour of the MUB flux of water as a function %of the timestep $dt$ used in the 3-point derivative. Each %panel shows a different Cartesian component of the flux for a %selected snapshot. The $x$-axis is in units of the simulation %step $\Delta t$. The picture shows that the code can handle %correctly even small values of $dt$. At the same time, it %shows that the non-linear effects due to high values of $dt$ %are present but, at least in the presented case, negligible, %allowing a $dt=2\Delta t$. } 
%    \label{fig:3p_econv}
%\end{figure}





%We can also discuss the effect of the \emph{velocity renormalization}. For each atom $t$ we can substitute its velocity $\bm V_t$ with $\bm V_t- \bm V^{\text{cm}}_{S}$, where $\bm V^{\text{cm}}_{S}$ is the velocity of the center of mass of the species of atom $t$. In theory, the resulting thermal flux can directly replace the non-renormalized flux in the GK-formulas. Still, the data analysis is much simpler since the renormalization technique decorrelates the energy flux from the mass one ( a spurious flux which should not contribute to thermal conductivity ) at the individual snapshot level, without having to run the whole trajectory. A longer discussion can be found in  \cite{Marcolongo2020}. In our examples, velocity renormalization does not change the qualitative behaviour of \cref{fig:3p_econv} or \cref{fig:3p_ecut} and, even if the renormalization might reduce the module of the flux by one order of magnitude removing spurious components, the oscillations with $dt$ remain small and within errorbars. For a more detailed discussion we remand the reader to \ref{sec:dt_ren_2p}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figure_reduced_spectrum.png}
    \caption{Reduced spectrum and logarithm of the reduced spectrum of a time series calculated with econv = $10^{-08}$ and dt = 3.0 rydberg atomic time units, twice the timestep used for the CP simulation, for a 64 water molecules system. Using smaller dt or smaller econv produces no appreciable difference. Note that the maximum frequency at which the spectrum can be estimated is the Nyquist frequency, defined as half of the sampling frequency. We computed the energy current once every 20 CP integration steps.}
    \label{fig:spectrum_high_low_comparison}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{figure_reduced_spectrum_high_low_precision_and_skip_low_freq.png}
%     \caption{Reduced spectrum of three different time series calculated with econv = $10^{-08}$ and econv = $10^{-11}$ and dt = 0.5, and one calculated with a third of the snapshots for a 64 water molecules system. There is no visible difference in the low frequency part of the spectrum, but the calculation with one third of the points costs one third of the computing time and it produces the same value of the thermal conductivity coefficient.}
%     \label{fig:spectrum_skip_comparison}
% \end{figure}



\subsection{Example of a thermal conductivity calculation}

As an example of a complete QE-Heat calculation, coupled with the SporTran tool for signal analysis, we report the results of a thermal conductivity calculation for water. For a complete description of the signal-analysis theory we refer to the works \cite{Baroni2020, Ercole2016} and to \cite{SporTran} for example notebooks and tutorials. We consider a 64 molecules water system at 600K. First,  the molecular dynamics trajectory was computed with the cp.x code using a cubic box with size of 12.43\AA  ~and an integration timestep of 3 Hartree atomic units, with a total length of 240ps. The power spectrum of the energy flux time series and the reduced power spectrum\cite{Bertossa2019}  are the key quantities needed to compute the thermal conductivity coefficient. The reduced power spectrum is used here to decorrelate the energy flux from spurious, non-diffusive signals, which are defined as signals not contributing to thermal conductivity. The high formation energies present in ab-initio computations may generate such components in the energy flux, which can be filtered out for example %either renormalizing the signal velocities snapshot by snapshot or a posteriori, after the \qeheat\ computation,
using the reduced power spectrum technique derived from the multicomponent formalism. For a longer discussion we refer to \cite{Marcolongo2020} and references therein. Here we filtered out the electronic density current and the ionic current, and the results are shown in fig.~\ref{fig:spectrum_high_low_comparison}. Using Sportran, the reduced power spectrum technique is transparently implemented and the thermal conductivity result can be produced with a single shell command specifying the parameters of the system and the file produced by the \qeheat\ code.   \\
\AM{\qeheat\ shows excellence stability properties as a function of the time-discretization parameter $dt$, which are show in Appendix . The value $dt=2\Delta t$, with $\Delta t$ being the Car-Parinello MD simulation timestep, is of particular interest because it would be beneficial in an on-the-fly computation, allowing to reuse the same wavefunctions computed in the MD simulation, neglecting the need for the recomputation of the scf cycles. In the Appendix we also show that,  at a fixed value of the self consistency threshold for convergence $econv$, the variance of the MUB estimator decreases with $dt$. Thus, it favourable, in order to control numerical noise, to choose $dt$ as large as possible, as long as the bias introduced by nonlinear effects is negligible. For these calculations,} we first investigated two values of $econv$, namely $10^{-8}$ and $10^{-11}$ Ry with a rather small $dt=0.5$ Rydberg atomic units. As expected, choosing the larger value raises the level of noise in the spectrum at very high frequencies where the magnitude of the spectrum is approximately zero, but with no effect on the thermal conductivity calculation. The final result of the computation, i.e. the thermal conductivity coefficient, is affected very weakly by this parameter, that on the contrary changes in a noticeable way the cost of the computation. In this case both computation gave $(1.00 \pm 0.10)$W/mK. Moreover we checked that using a $dt$ that is equal to the integration timestep of the Car-Parrinello simulation and $econv$= $10^{-8}$ produces the same spectrum with no noticeable differences and the same thermal conductivity coefficient: in this case we had $(0.98 \pm 0.09)$W/mK. This calculation is shown in fig.~\ref{fig:spectrum_high_low_comparison}.
We also stress that it is not necessary to compute the energy flux for every single step of the molecular dynamics trajectory, in order to avoid unneeded wastes of computer time. In order to sample correctly the spectrum, it is sufficient to sample the signal such that for any frequency larger than the Nyquist frequency the energy flux spectrum is very small. In the signal processing literature the Nyquist frequency is defined as half of the sampling frequency. In our example we used a Nyquist frequency of $345~$THz that means sampling every 60 units of time in Hartree atomic unit. In general we warn the user to do an estimate of the sampling frequency needed before starting the \qeheat\ computation, for example by calculating the power spectrum of the atomic velocities and estimating a frequency $f_v$ at which the velocity spectrum has gone to zero. Since the energy flux is cubic in the velocities, we suggest a Nyquist frequency larger than $3f_v$. We also suggest a conservative approach and a-posteriori checks on the computed spectra, checking that the computed spectra vanish at the Nyquist frequency. According to our experience, the overall cost of a \qeheat\ calculation is often of the same order of magnitude of the full Car Parrinello molecular dynamics simulation even if the \qeheat\ computation can be trivially parallelized. The data analysis with SporTran adds a negligible computational cost.

